Control What You Include! Server-Side Protection against Third Party Web Tracking

Third party tracking is the practice by which third parties recognize users accross different websites as they browse the web. Recent studies show that 90% of websites contain third party content that is tracking its users across the web. Website developers often need to include third party content in order to provide basic functionality. However, when a developer includes a third party content, she cannot know whether the third party contains tracking mechanisms. If a website developer wants to protect her users from being tracked, the only solution is to exclude any third-party content, thus trading functionality for privacy. We describe and implement a privacy-preserving web architecture that gives website developers a control over third party tracking: developers are able to include functionally useful third party content, the same time ensuring that the end users are not tracked by the third parties.

==> discussions.tex <==
\section{Discussion}
\subsection{Stateless Tracking Prevention}
Even though this work did not address stateless tracking, there are some interesting side-effects worth noting. 
The redirection to the middle party anonymizes the real IP addresses of users to third parties.
Some stateless tracking APIs such as \code{window.navigator, window.screen, HTMLCanvasElement} can be easily removed or randomized from the context for the webpage to mitigate stateless tracking.
%\begin{itemize}
% \item The redirection to the middle party anonymizes the real IP addresses of users to third parties.
% \item Some stateless tracking APIs such as \code{window.navigator, window.screen, HTMLCanvasElement} can be easily removed from the context for the webpage to mitigate stateless tracking.
%\end{itemize}
We leave this for a future work.

\subsection{Towards Complying with Privacy Standards and Regulations}
We argue that this architecture can serve as a base for websites to comply with upcoming anti-tracking regulations and standards.
The logic of the website is kept unchanged. But the rewrite server is instructed in order to take the necessary actions for users privacy.

\subsection{Anti-Tracking standards}
With the prevalence of third party tracking on the web, we have shown the challenges that a developer will face towards mitigating that.
The sandbox attribute for iframes help prevent access to security-sensitive APIs. As tracking has become a hot concern, we suggest that 
similar mechanisms can help first party websites tackle third party tracking. The sandbox attribute can for instance be extended with 
specific values to tackle tracking. Even though sandboxing has the interesting side-effect of 

==> solution.tex <==
\section{Privacy-preserving Web Architecture}
\label{sec:solution}

To help web developers keep their promises of non-tracking and still include 
third-party content in their web applications, we propose a new Web application 
architecture with the capability to: 1) automatically rewrite all the  third party 
\emph{in-context} content of a Web application, 2) redirect the third party HTTP 
requests issued by the \emph{in-context} content, and 3) remove/disable known 
\emph{statefull} tracking mechanisms (see Section~\ref{sec:background}) 
for such third party content and requests. 

 \begin{figure}
  \includegraphics[width=1\textwidth]{images/p_architecture}
  \caption{Privacy-Preserving Web Architecture}
  \label{fig:p_architecture}
  \end{figure}
  
Figure~\ref{fig:p_architecture} provides an overview of 
our web application architecture, that introduces two new 
components that are fully controlled by the website owner:
%

{\bf Rewrite Server (Section~\ref{sec:rewrite})} acts like a reverse 
proxy\footnote{\url{https://en.wikipedia.org/wiki/Reverse_proxy}} for the original web pages. 
It rewrites the web pages in such a way that all the %\emph{controllable} 
third party requests (which are possible to control, see Section~\ref{sec:problem}) 
are redirected through the \MPS\ before reaching the intended third party server. 

{\bf Middle Party Server (Section~\ref{sec:middle})} is at the core 
of our solution since it redirects all the third party 
requests to the third party server and removes stateful tracking. 
On one hand, it hides the third party destination from the browser, and therefore prevents the 
browser from attaching third party HTTP cookies to such requests. 
Because the browser will still attach some tracking information to the requests, such as ETag, and 
Referer headers, Middle Party Server will also remove this informaiton when forwarding the 
requests to the third party.
On the other hand, the Middle Party Server prevents both types of stateful tracking: 
passive and active. For passive tracking (via HTTP headers), the server removes 
tracking identifiers set by the third party, such as HTTP cookies and  Etag, 
before forwarding the response back to the browser.
For active tracking (via JavaScript code execution), \MPS\ 
rewrites web pages before forwarding it back to the browser:
it injects JavaScript code that prevents access to tracking APIs, 
and cleans browser storages that are often used for tracking.
%and APIs used to exchange tracking information between \code{in-context} and \code{cross-context} cooperating third party 
%contents.
%The rewritting helps mitigate \code{cross-context} third party tracking.




\subsection{Rewrite Server}
\label{sec:rewrite}

The goal of the \RS\ is to rewrite the original content of the requested wepages
in such a way that all the \emph{in-context} third party content will be redirected 
to the \MPS. It consists of three main components: static HTML rewriter for HTML pages, 
static CSS rewriter and JavaScript injection component. Into each webpage, 
we inject a JavaScript code that insures that all the dynamically generated 
third party content is redirected to the \MPS. 

%\begin{figure}[!tp]
%  \includegraphics[width=1\textwidth]{images/rserver}
%  \caption{Details of The Rewrite Server}
%  \label{fig:rserver}
%\end{figure}

%Figure~\ref{fig:rserver} presents the architecture of the Rewrite Server.  
%\subsubsection{Web Pages Rewriter.}

\subsubsection{HTML Page Rewriter} rewrites the URL of static third party contents embedded in original web pages in order to redirect them to the \MPS. 
For example, the following inclusion of a third-party script from \code{http://third.com} domain 
\code{<script src="http://third.com/script.js"></script>}
is written to
\code{<script src="http://middle.com/?src=http://third.com/script.js"></script>}. 
The same process is followed for other static third party contents.

\subsubsection{CSS File Rewriter} rewrites CSS files in order to ensure that all 
the third party contents, like images and fonts, are redirected though the \MPS.
%CSS files are a particular case, because they can further embed third party images and fonts. 
%That's why we write them, just as we do with static third party contents in original web pages.
We present an example of CSS rewriting in the Appendix.

\subsubsection{JavaScript Injection}
\NB{This subsubsection is for Francis to explain}

{Dynamic Content Handler.}
Dynamic contents are those injected by scripts client-side. In order to handle those, we inject in original page a script that controls APIs used to inject dynamic contents.
The part of this script that redirect dynamically injected scripts tag is:
\begin{verbatim}
  HTMLScriptElement.prototype.sat = HTMLScriptElement.prototype.setAttribute;
  HTMLScriptElement.prototype.setAttribute = function(at, nv){
      if(at === "src"){
        this.sat(at, handleURL(nv, 'src'));
      }else{
        this.sat(at, nv);
      }
  };
  Object.defineProperty(HTMLScriptElement.prototype, 'src', {
    set: function(nv) {this.setAttribute('src', nv)},
    configurable: false
  });
\end{verbatim}
where \code{handleURL} is a function that rewrites the URL in case it is a third party URL, prefixing it with the URL of middle party, as we have done with static third party contents.

The following code shows how AJAX requests are redirected.
\begin{verbatim}
XMLHttpRequest.prototype.op = XMLHttpRequest.prototype.open;
XMLHttpRequest.prototype.open = function(m, u, b, o, t) {
  this.op(m, handleURL(nv, 'src') + '&su=' + btoa(document.location.origin), b, o, t);
};
\end{verbatim}

{Anti-Tracking Handler.}
Since statefull tracking is infeasible for \code{in-context} third party content, the anti-tracking handler injects a script that prevent access to stateless tracking APIs.
They include \code{window.navigator, window.screen, navigator.plugins, document.fonts}, \code{HTMLCanvasElement.toDataURL()},\\ \code{HTMLCanvasElement.toBlob(), document.URL, document.location, } etc.
The following snippet of code removes the navigator object from the context of the web page.
\begin{verbatim}
 (function(window) {
  delete window.navigator;
  delete window.screen;
  }(window));
\end{verbatim}

The other one removes methods for canvas fingerprinting.
\begin{verbatim}
    Object.defineProperty(HTMLCanvasElement.prototype, 'toDataURL', {
      get: function() {return function(){return Math.random()}},
      configurable: false, editable: false
    });
    
    Object.defineProperty(HTMLCanvasElement.prototype, 'toBlob', {
      get: function() {return function(cb, mtype, qa){cb(Math.random())}},
      configurable: false, editable: false
    });

\end{verbatim}

It also controls inter-frame communications.  
In order to send a message to a \code{cross-context} script, an \code{in-context} script invokes the \it{postMessage} API, providing two arguments: the message to be sent and the targetted \code{cross-context}, identified by its URL. 
Since the target of messages is known, we check if it is a \code{cross-context}. In this case, the message is discarded.
Conversely, in order for an \code{in-context} script to receive \code{cross-context} scripts messages, it has to register an event listener for those messages. 
Once a message is received, we check its origin. If the message was sent by a third party context, we discard it, so that it does not reach the targetted script.

\begin{verbatim}
 Code for preventing inter-frame communications.
\end{verbatim}


\subsubsection{Content Security Policy.}
A CSP header is injected in all original web pages. It purposes is to prevent malicious third party content from bypassing the redirections to the middle party.
If a malicious script managed to bypass the rewritting restrictions, it could make a request directly to the malicious third party server without going through the middle party.
This could happen if there were no CSP installed on the web page. 
The CSP injected on all web pages is rather simple. Since all third party requests now go through the middle party, the CSP whitelists only two origins: the middle party and the original server.
\begin{verbatim}
Content-Security-Policy: default-src 'self' m.com; frame-ancestors 'self' m.com; 
\end{verbatim}
This CSP can be customized by the first party owner in order to handle tracking based on plugins. 
To forbid plugins within all web pages, one can add to the previous CSP the following directive \code{object-src 'none'}. 
To allow pluings from the same domain, one can use the following directive instead: \code{object-src 'self'}.




  
\subsection{Middle Party}
\label{sec:middle}


Because of the SOP restrictions, we know exactly how statefull tracking can happen and how we can prevent them. 
\subsubsection{\code{In-Context} Statefull Tracking.}
The redirection to the middle party successfully prevents tracking based on the following mechanisms:
  \begin{itemize}
   \item \emph{Cookie, Set-cookie} 
   \item \emph{Etag}
   \item \emph{Last-Modified, If-Modifed-Since}
   \item \emph{Browser storages} cannot be used to track users.
   \item \emph{Referrer}
   \item \emph{Plugins Storages}: with the use of CSP, we have restricted plugins that can be loaded only to those that come from the developer own server. This prevents tracking based on them.
  \end{itemize}
However, it is not possible to prevent the following mechanisms: 
  \begin{itemize}
   \item \emph{Origin}: This is used to perform CORS requests. If the developer does not fetch AJAX contents on third party servers, it can customize the middle party to remove this header in third party requests.
   \item \emph{window.location, document.location}: those mechanisms can still be used to identify the web application. However, since the third parties cannot identify the user, tracking is not possible.
  \end{itemize}
  
 The middle party is a trusted third party server fully controlled by the website owner where third party requests are redirected.
    \begin{figure}[!tp]
    \includegraphics[width=1\textwidth]{images/mparty}
    \caption{Details of Middle Party Server}
    \label{fig:mparty}
    \end{figure}
Figure~\ref{fig:mparty} gives details of its different components.

\subsubsection{Request Tracking Information Handler.}
It intercepts third party requests sent by browsers, removes passive tracking information, and forwards them to the third party.
The tracking information which are removed include \code{cookie, etag, referrer, if-modified-since, user-agent}.

\subsubsection{Response Tracking Information Handler.}
It removes tracking information that are attached to third party responses. This include \code{set-cookie, etag, last-modified}.
It also rewrite redirection URLs in order to make them redirect back to the middle party. a \emph{Location} HTTP header \code{Location: http://t.com/} is 
changed to \code{Location: http://m.com/?src=http://t.com/}

\subsubsection{CSS Files Handler.}
This component works exactly the same way as that of the rewrite proxy. It redirect background images and fonts to the middle party.

\subsubsection{Iframes Handler.}
\label{sec:iframehandler}

Rewritting third party \code{cross-context} contents as done in~\ref{sec:iframehandler} with sanbboxing helps mititage the following tracking mechanisms:
\begin{itemize}
 \item \emph{Referrer} for application identification
 \item \emph{Access to Browser and Plugins storages}
\end{itemize}

However, user information are still transmitted by browsers, such as \emph{Cookie, Set-Cookie, Etag, Last-Modified, If-Modified-Since, etc.}. 
Moreover, if the iframe or window are dynamically created by third party scripts, application identification information could be transmitted to \code{cross-context} third party contents in the form
of URL arguments.

Nonetheless, this mitigation becomes very effective if the user has enabled third party cookies blocking.



We has already argued that being able to identify a user is not sufficient in 
tracking him. Since \code{cross-context} third party contents are out of control for a web developer.
In order to mititage \code{cross-context} third party tracking, we perform the following actions.
When the middle party receives requests to fetch \code{cross-context} containing the URL of the third party (\code{http://t.com/}, it does not forward the request directly to the middle party.
It returns the following response:
\begin{verbatim}
 <html>
  <body>
    <a href="http://t.com" rel="noopener noreferrer" target="_self"></a>
    <script>
      document.getElementsByTagName("a")[0].click();
    </script>
  </body>
 </html>
\end{verbatim}
The response is also sent along with the following CSP header
\begin{verbatim}
 Content-Security-Policy: sandbox allow-scripts;
\end{verbatim}

When the browser renders this response, the script gets executed, and the original third party iframe is loaded, with many limitations:
\begin{itemize}
 \item First, the third party cannot identify the origin of the request, since no referrer header is sent with the request.
 \item User identification is possible but limited to stateless tracking and stateull tracking user identification information transmitted by the browser. Browser and Plugins storages cannot be accessed. 
 \item Plugins are blocked.
\end{itemize}
